Spectroscopy Approaches for Food Safety Applications: Improving Data Efficiency Using Active Learning and Semi-Supervised Learning

The past decade witnesses a rapid development in the measurement and monitoring technologies for food science. Among these technologies, spectroscopy has been widely used for the analysis of food quality, safety, and nutritional properties. Due to the complexity of food systems and the lack of comprehensive predictive models, rapid and simple measurements to predict complex properties in food systems are largely missing. Machine Learning (ML) has shown great potential to improve classification and prediction of these properties. However, the barriers to collect large datasets for ML applications still persists. In this paper, we explore different approaches of data annotation and model training to improve data efficiency for ML applications. Specifically, we leverage Active Learning (AL) and Semi-Supervised Learning (SSL) and investigate four approaches: baseline passive learning, AL, SSL, and a hybrid of AL and SSL. To evaluate these approaches, we collect two spectroscopy datasets: predicting plasma dosage and detecting foodborne pathogen. Our experimental results show that, compared to the de facto passive learning approach, AL and SSL methods reduce the number of labeled samples by 50% and 25% for each ML application, respectively.

==> abstract.tex <==

\begin{abstract}

The past decade witnesses a rapid development in the measurement and monitoring technologies for food science. Among these technologies, spectroscopy has been widely used for the analysis of food quality, safety, and nutritional properties. Due to the complexity of food systems and the lack of comprehensive predictive models, rapid and simple measurements to predict complex properties in food systems are largely missing. Machine Learning (ML) has shown great potential to improve classification and prediction of these properties. However, the barriers to collect large datasets for ML applications still persists. 
%With the rapid development of computational capabilities and big data technologies, Machine Learning (ML) has been applied to various fields, achieving state-of-the-art performance. To train an ML model, collections of labeled samples are often prerequisites. Typically, unlabeled samples can be collected in a large quantity and cheap way (e.g., images of vineyards). In contrast, the sample annotation process (e.g., the number of grapes in each image view) is costly and time-consuming as humans effort and in-field experiments are usually involved in annotating samples. 
In this paper, we explore different approaches of data annotation and model training to improve data efficiency for ML applications.  Specifically, we leverage Active Learning (AL) and Semi-Supervised Learning (SSL) and investigate four approaches: baseline passive learning, AL, SSL, and a hybrid of AL and SSL. To evaluate these approaches, we collect two spectroscopy datasets: predicting plasma dosage and detecting foodborne pathogen. Our experimental results show that, compared to the \textit{de facto} passive learning approach, AL and SSL methods reduce the number of labeled samples by 50\% and 25\% for each ML application, respectively.


\end{abstract}



==> active_learning.tex <==
\subsection{Active Learning: A Primer}
\label{sect:active_learning}

AL, also known as query learning/optimal experimental design, is a sub-field of machine learning, which studies ML models that improve with experience and training~\citep{burr_active_learning_book}.
Compared with passive learning, AL considers the ``usefulness'' of unlabeled samples for the current ML model. It strategically selects unlabeled samples for annotation to improve data efficiency for ML model training.



Algorithm \ref{alg:pool-based} shows the workflow of the AL-based data annotation. $\mathcal{U}$ and $\mathcal{L}$ is the set of unlabeled samples and labeled samples, respectively (line 1-2). The ML model, denoted by $\theta$, is trained on the labeled sample set $\mathcal{L}$ (line 4). The following unlabeled sample, denoted by $x^*$, is selected that has the highest utility measure according to the currently trained model $\theta$ (line 5). Then, the experiment is conducted for $x^*$, which obtains its ground-truth label by human experiments, denoted by $y^*$ (line 6). Since the label for $x^*$ is obtained, $x^*$ is removed from the pool of unlabeled samples $\mathcal{U}$, and $x^*$ along with its label $y^*$ is added to the set of labeled samples $\mathcal{L}$ (line 7). The whole process repeats until the trained model $\theta$ has a satisfactory accuracy or does not improve with more labeled samples. 


The utility measure is essential for AL algorithms. There are various utility measures to estimate the usefulness of an unlabeled sample to the ML model. They mostly leverage the probability of the current ML model classifying an unlabeled sample $x$ to class $y$, i.e., $P_{\theta}(y|x)$. We introduce two categories of utility measure methods of AL: uncertainty-based sampling~\citep{al_uncertainty} and minimizing expected errors~\citep{al_expected_errors}.


\subsubsection{Uncertainty Sampling based Active Learning}




The premise of uncertainty sampling is that we can avoid annotating samples that the ML model is confident about and focus instead on the unlabeled samples that confuse the ML model. Least confident and entropy are the most used metrics for measuring the uncertainty of unlabeled samples. 


\begin{itemize}
    \item \textit{Least Confident}. For an unlabeled sample $x$, we can apply the currently trained ML model on it, which outputs the probability of the sample belonging to class $y$, i.e., $P_{\theta}(y|x)$, where $y = 1, 2, ..., C$ and $C$ is the total number of classes for classification. Let's denote by $\hat{y}$, the class that is most likely for the unlabeled sample $x$, i.e., $\hat{y} = \argmax_y P_{\theta}(y|x)$. The confidence of the current model for the sample $x$ is thus $P_{\theta}(\hat{y}|x)$. The unlabeled sample with the least confidence is selected for annotation, that is,
\begin{equation}
    x_{LC}^* = \argmax_x 1 - P_{\theta}(\hat{y} | x)
    \label{equ:least_confident}
\end{equation}     

\item \textit{Entropy}. Entropy is an often-used metric for quantifying the uncertainty of a distribution. For an unlabeled sample $x$, its entropy is calculated as $-\sum_y P_{\theta}(y | x) \cdot \log P_{\theta}(y | x)$, which is over the distribution of classes $y$ for $x$. The entropy-based uncertainty sampling selects the sample with the maximum entropy, i.e., 
\begin{equation}
    x^*_E  = \argmax_x -\sum_y P_{\theta}(y | x) \cdot \log P_{\theta}(y | x)
    \label{equ:entropy}
\end{equation} 
\end{itemize}


\subsubsection{Minimizing Expected Error based Active Learning}

This category of AL algorithms aims to select samples to directly increase the model accuracy without relying on the assumption between the sampling strategy and the model performance (e.g., the ML model can avoid annotating confident samples as in the uncertainty sampling). Since the ground-truth label of an unlabeled sample $x$ is not available without experiment and annotation, the model accuracy by adding the sample $x$ and its label to the training set is unknown. Nonetheless, we can estimate the expected model accuracy when the sample $x$ is added for training, thus selecting a sample that minimizes the expected error of the current ML model. 


Assume that the unlabeled sample $x$ belongs to the class $y$. 
%We can update the model $\theta$ by adding the unlabeled sample $x$ and its imaginary label $y$. 
Let's denote by $\theta^+$ the updated ML model by adding the sample $x$ and its imaginary label $y$ to the training set. Then, the expected prediction error of the model $\theta^+$ can be estimated by applying $\theta^+$ to all unlabeled samples in $\mathcal{U}$, i.e., $\sum_{x' \in \  \mathcal{U}} 1 - P_{\theta^+}(\hat{y}|x')$, where $1 - P_{\theta^+}(\hat{y}|x')$ is the prediction error for the unlabeled sample $x'$. Since the probability that $x$ belongs to class $y$ is $P_\theta(y|x)$, the expected prediction error of selecting the unlabeled sample $x$ for annotation is $\sum_y P_{\theta}(y|x) \left[\ \sum_{x' \in \  \mathcal{U}} 1 - p_{\theta^+}(\hat{y}|x') \right]$. Correspondingly, Eq.~(\ref{equ:expected_prediction_error}) formulates the sampling strategy that minimizes the expected prediction error. 
\begin{equation}
    x_{EPR}^* = \argmin_x \sum_y P_{\theta}(y|x) \left[\ \sum_{x' \in \  \mathcal{U}} 1 - p_{\theta^+}(\hat{y}|x') \right]
    \label{equ:expected_prediction_error}
\end{equation}
 
An alternative to minimizing the expected prediction error is minimizing the expected log-loss error. Log-loss error is the \textit{de facto} loss function for training a classification model. Therefore, minimizing the expected log-loss error has a strong connection with ML model training. By replacing the prediction error $1 - p_{\theta^+}(\hat{y}|x')$ in Eq.~(\ref{equ:expected_prediction_error}) with the log-loss error $-\sum_{y'} P_{\theta^+}(y' | x') \cdot \log P_{\theta^+}(y' | x')$,  Eq.~(\ref{equ:expected_logloss_error}) formulates the sampling strategy of minimizing the expected log-loss error. 
\begin{equation}
    x_{ELR}^* = \argmin_x \sum_y P_{\theta}(y|x) \left[\ \sum_{x' \in \  \mathcal{U}} -\sum_{y'} P_{\theta^+}(y' | x') \cdot \log P_{\theta^+}(y' | x') \right]
    \label{equ:expected_logloss_error}
\end{equation}





 
\begin{algorithm}[!t]
\SetAlgoLined

$\mathcal{U}$: set of unlabeled samples $\{x^{(u)}\}_{u=1}^U$

$\mathcal{L}$: set of labeled samples $\{\langle x, y\rangle^{(l)}\}_{l=1}^L$

\For{$t = 1, 2, ...$ }{
    $\theta = \textbf{train}(\mathcal{L})$\\
    select $x^* \in \mathcal{U}$, the unlabeled sample of the highest \emph{utility measure} according to the model $\theta$\\
    conduct experiment for $x^*$, which obtains its label $y^*$ \\
    remove $x^*$ from $\mathcal{U}$, and add $\langle x^*, y^* \rangle$ to $\mathcal{L}$ 
}
\caption{Selection of unlabeled samples for annotation in active learning.}
\label{alg:pool-based}
\end{algorithm}

==> conclusion.tex <==
\section{Conclusion}


In this paper, we target
data efficiency of ML applications for spectroscopy analysis in food science.  To mitigate the annotation cost by reducing the number of labeled samples, we explore different approaches of data annotation and model training: passive learning, active learning, semi-supervised learning, and the hybrid of active learning and semi-supervised learning. We evaluate these approaches with our two datasets and find that advanced approaches can greatly improve data efficiency for ML model training. These approaches are general and thus can be applied to various ML-based food science research. 





==> dataset.tex <==
\subsection{Dataset}
\label{sect:dataset}

We collect two spectroscopy datasets in food science. One dataset is to predict the plasma dosage and the other one to detect the foodborne pathogen. Our datasets are diverse and representative in terms of data structures (2D vs 1D spectroscopy) and tasks (multi-class classification vs binary classification). In addition, we use different ML models for these two datasets. 


\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{image/dataset.png}
    \caption{Two datasets are used in our experiments. The first row shows the plasma dosage classification dataset where (A) is the sample distribution of the four classes, (B) is the clustering result, and (C) illustrates a sample for each class. The second and the third row shows the pathogen detection dataset. (D) is the sample distribution where 24 samples are from T7 infected E. coli, and 48 control samples (24 T7-only and 24 E. coli-only samples), (E) is the clustering result, and (F) depicts a sample for the T7 infected E. coli, a sample for the T7-only, and a sample for the E. coli-only, respectively. }
    \label{fig:dataset}
\end{figure}

\subsubsection{Dataset 1: Plasma Dosage Classification}

As an emerging nonthermal processing technology, plasma is highly effective in inactivating various types of food pathogens in solution as well as on food contact surfaces~\citep{plasma_review}. One of the main goals of our dosage classification dataset is to evaluate whether the plasma dosage can be predicated using the Fourier-Transform Infrared Spectroscopy (FTIR) spectral response of DNA sample exposed to the plasma treatment. The dataset was obtained by subjecting substrate to plasma treatment at various dosage levels and characterizing biochemical changes of substrate with FTIR. The data comprise aborbance intensities at various IR wavenumbers of the substrate under plasma treatment.



%As an emerging nonthermal processing technology, plasma has drawn lots of attention in the food industry. One of the main goals of our dosage classification dataset is to evaluate whether the plasma dosage can be predicated using the frequency reflectance change of the substrate exposed to the plasma treatment. 

%In particular, Chitosan-DNA substrate was used. 
%The reflectance spectra were characterized with the Fourier transform infrared (FTIR) spectroscopy. 
%Vibrational spectroscopy such as FTIR can provide a molecular fingerprint that can be used for evaluating the impact of the oxidants on molecules \citep{ftir}.
%Plasma activated water was produced by exposing deionized water (DI water) to plasma jet. %The distance between the end of plasma nozzle and the water surface was constant at 5 cm. DI water of 200 mL was filled in a 1 L glass beaker and activated by plasma for 2min, 5 min or 10 min. 
%Chitosan-DNA substrate was prepared by coating Chitosan-DNA bilayers on stainless steel coupon. 10 mg/ml Salmon sperm DNA 40 ul was added to stainless steel and dried in room temperature. Then, another layer of chitosan dissolved in sodium acetate/acetic acid pH 4.76 was spread on top of DNA layer and dried at room temperature. DNA was recovered after plasma treatment and spotted on anodisc membranes (0.2 mm pore size, 13 mm OD) and dried with filtration system. FTIR spectra were collected using IRPrestige-21 FTIR spectrometer (Shimadzu Co., Kyoto, Japan). The anodisc filter containing a uniform thin layer of DNA was placed directly on the diamond crystal cell of attenuated total reflectance (ATR). 


Our 1-D dosage classification dataset categorizes the plasma dosage into four classes, where classes 1, 2, 3, and 4 represent plasma injection of 0 minutes, 2 minutes, 5 minutes, and 10 minutes, respectively. 
Fig.~\ref{fig:dataset}(A) shows the number of samples of each class. In total, we collect 114 samples, where classes 1, 2, 3, and 4 have 27, 27, 30, 30 samples, respectively. To study the sample distribution over the feature domain, we apply K-Means~\citep{k_means} to group samples into 4 clusters. Fig.~\ref{fig:dataset}(B) shows the clustering result. It indicates that the class 2 and the class 3 samples are well clustered, while many of the class 4 samples are located within cluster 2 and cluster 3 (a PCA visualization is given in Fig.~\ref{fig:sample_selection}). Fig.~\ref{fig:dataset}(C) illustrates a sample for each class. Each sample contains 1868 values representing the intensity of the IR frequency reflectance in the range of 400 Hz to 4000 Hz with a step of 2 Hz. We use our dosage classification dataset to train a multi-class classification ML model.    



\subsubsection{Dataset 2: Foodborne Pathogen Detection}

%Detection of the bacterial foodborne pathogen is one of the critical processes in the food and agricultural industry as it ensures the safety of food products before distribution and also reduces the risk of foodborne illness outbreak~\citep{pathogen_review}.  The dataset for pathogen detection was obtained by using bacteriophage for infection and lysis of the target bacterial pathogen in food samples. The fluorescence spectroscopy was then used to acquire the fluorescence Excitation Emission Matrices (EEM)~\citep{t7phage20chemical} of each sample. The data comprise fluorescence emission intensities at several pairs of excitation/emission wavelengths. 
%We use the pathogen detection dataset to train a binary classification ML model. 

Detection of the bacterial foodborne pathogen is one of the critical processes in the food and agricultural industry~\citep{pathogen_review}. It ensures the safety of food products before distribution and reduces the risk of a foodborne illness outbreak. Among various types of bacteria, E. coli has been used as an indicator of the fecal contamination and poor sanitary quality of food and water~\citep{t7phage83aem}. 
%The development of a rapid and sensitive E. coli detection method is required to improve the detection efficiency and reduce the cost and time of the operation.
T7 bacteriophage or T7 phage has been used as a tool for E. coli detection as it specifically infects E. coli cells results in bacteria cell lysis and release of the cell components along with the amplified T7 phage progenies~\citep{t7phage20plosone}. Therefore, bacterial cell lysis and T7 phage amplification can indicate E. coli contamination in the samples. Fluorescence EEM spectroscopy is an analytical technique providing multidimensional information~\citep{t7phage20chemical} that has been used to detect organic materials, including bacterial cells~\citep{eem20water}. 

%Spinach wash water samples were inoculated with E. coli followed by enrichment before adding T7 phage for infection for 1 hour. After infection, the samples were collected and washed with sterile phosphate buffer saline and resuspended in Milli-Q water. The EEM spectra of the resuspended samples were collected with the wavelength range of 250–400 nm for excitation and 260–450 nm for emission with 5-nm increments. The obtained emission intensities will be subtracted with the emission intensities of the milli-Q water. The controls were spinach wash water samples with E. coli without T7 phage and spinach wash water with T7 phage without E. coli. 

%The total of 72 EEM spectra were collected, 24 for samples with both E. coli and T7 and 24 for each type of control.
%We are asked to distinguish the samples containing T7 phage infected E. coli from 2 types of controls which are samles containing only T7 phage without E. coli (type 1) and E. coli without T7 phage (type 2). 

We explore whether 2-D EEM spectroscopy can detect the change of the physical and chemical properties of the samples due to the T7 infection of E. coli. 
The EEM spectra of the resuspended samples were collected with the wavelength range of 250–400 nm for excitation and 260–450 nm for emission with 5-nm increments.
Fig.~\ref{fig:dataset}(D) illustrates the sample distribution, where 24 samples contain T7 phage infected E. coli and 48 control samples (24 T7-only samples and 24 E. coli-only samples).  Fig.~\ref{fig:dataset}(E) shows the result of grouping the samples into 2 clusters using K-Means. It indicates that the samples of the pathogen detection dataset cannot be easily separated, with 41.67\% target samples are wrongly classified to the cluster of the controls. Fig.~\ref{fig:dataset}(F) visualizes one sample for the T7 infected E. coli, the T7-only sample, and the E. coli-only sample, respectively. The example samples are visually similar to each other.  In the heat maps, we take the logarithm of the frequency intensity at each frequency pair of the excitation and emission wavelength.  In total, we collect 72 samples, and each sample includes 744 numbers representing the fluorescence response for the excitation-emission pairs. We use our pathogen detection dataset to train a binary-classification ML model. 

% \subsubsection{Dataset Summary}

% \huanle{move to Section 2.3}

% We select two spectroscopy datasets for experiments because they are commonly used in the food and agriculture sectors for monitoring quality, safety, and production of food. Our datasets are diverse and representative. The plasma dosage classification dataset is 1-D input, while the foodborne pathogen detection dataset is 2-D input. In addition, they target different tasks: one for multi-class classification and the other one for binary classification, and we apply different ML models for them. 

==> discussion.tex <==
\section{Discussion}

We explore different approaches of data annotation and model training to improve data efficiency for ML applications. In this section, we discuss practical considerations in applying these advanced approaches.  

\subsection{Practicability of Advanced Approaches}


The passive learning approach has been adopted for the majority of projects. An essential question is whether the other more advanced approaches can be effectively and efficiently applied for new projects, considering the overheads of implementing these approaches. We argue that when the annotation process is costly, the benefits of the reduced number of labeled samples overweigh the implementation overheads. In fact, AL and SSL have been successfully applied to many domains~\citep{ssl_drug,al_material, ssl_material,opex20nature,ssl_biology}. For example,  the medicine industry applies AL to discover antagonists for dopamine $D_4$~\citep{drgu_d4} and CXC-chemokine~\citep{drgu_chemokine}, among the estimated range of $10^{30}$-$10^{60}$ drug-like molecules~\citep{al_drug}. In food systems, development of AL and SSL methods can aid in addressing challenges of obtaining labeled samples for ML models as many of these labeled samples in food safety applications require both resources and extended time. 


\subsection{Determining the Optimal Approach}

We introduce three advanced approaches of data annotation and model training and compare their performance with the passive learning approach. Generally, the passive learning approach performs the worst compared to the other three approaches. However, there is no guarantee on which approach works best \textit{a priori}. For example, the hybrid approach works exceptionally well for the dosage classification dataset, while the AL approach works the best for the pathogen detection dataset. Nonetheless, there are several rules of thumb drawn from the community~\citep{burr_active_learning_book,semi_supervised_learning_survey20ML}. 
Based on our experience, we suggest the following approach selection procedure: (1) If the data samples are poorly clustered, SSL is not expected to work. In this case, we advocate the AL approach. To decide whether data samples can be clustered, we can either apply PCA visualization or k-means clustering algorithms~\citep{k_in_k_means} to check whether the number of clusters is close to the number of classes for classification. (2) If the data samples are well-clustered, we suggest the hybrid approach that leverages both AL and SSL. 


\subsection{Determining the Optimal Sampling Strategy in Active Learning}

There are a great variety of sampling strategies available for AL~\citep{burr_active_learning_book}. 
Although it is not possible to obtain a universally good AL sampling strategy~\citep{greedyactive04nips}, we have demonstrated that by using simple sampling strategies such as uncertainty-based sampling, we achieve better data efficiency than the passive learning approach. Simple sampling strategies based on uncertainty and disagreement are recommended if the domain knowledge about the samples and the problems are not available~\citep{burr_active_learning_book}. On the other hand, incorporating domain knowledge into AL can further improve data efficiency. For example, \cite{alice20emnlp} proposes an expert-in-the-loop AL framework that utilizes language explanations from domain experts to iteratively distinguish misleading breeds of birds, which outperform baseline models that are trained with 40\%-100\% more training samples. Automatic selection of sampling strategies has also been extensively studied, e.g., \citep{al_learning_15aaai} and~\citep{alFromData17nips}.


In our experiments, we warm start the initial ML model by randomly selecting and training 40 samples for the dosage classification dataset and 25 samples for the pathogen detection dataset. Another common practice is to switch between random sampling (for exploration) and AL sampling strategy (for exploitation). For example, \cite{opex20nature} train a predictive ML model of gene expression with 44\% fewer data by consecutive switching between random sampling and mutual information based AL sampling strategy.  


\subsection{Determining the Optimal Pseudo-Labeling Method in Semi-Supervised Learning}

In addition to the self-training and the label spreading methods, semi-supervised learning includes many other methods such as co-training, boosting, and perturbation-based~\citep{semi_supervised_learning_survey20ML}. Similar to AL, SSL does not guarantee better data efficiency than the passive learning approach~\citep{hurt_ssl}. Nonetheless, our experiments demonstrate that simple pseudo-labeling methods such as self-training and label spreading can greatly improve the model accuracy when the underlying samples can be well-clustered and the number of labeled samples are small. 
Recent advances in SSL show promising results of the perturbation-based semi-supervised neural networks, which empirically and consistently outperforms the passive learning approach~\citep{semi_supervised_learning_survey20ML}. We leave it as future work to evaluate the perturbation-based methods. 


\subsection{Extension for Regression Problems}

Both classification and regression are common problems. In this paper, we use classification to illustrate different approaches of data annotation and model training.  Although methods designed for classification may not be applied to regression problems, we expect our main conclusion to remain valid for regression problems; that is, advanced approaches can help improve data efficiency for model training compare to the passive learning approach. There are many existing works solving regression problems in AL and/or SSL~\citep{al_regression,ssl_regression}, which we will explore in our future work. 

\subsection{Applicability for Diverse Applications in Food Quality, Traceability and Safety}
% Spectroscopic analysis has been widely used for the analysis of food quality, safety, and nutrition in food science. We collect two spectroscopy datasets in our experiments, which show promising results of using advanced approaches. We believe that AL and SSL can also improve data efficiency for other food science problems. .........

The spectroscopy measurement approaches selected for this study represent two distinct spectral methods, namely IR spectroscopy and fluorescence spectroscopy. IR spectroscopy has been proposed for diversity of applications in food quality~\citep{food_quality}, traceability~\citep{food_traceability} and food safety~\citep{food_safety}. These diversity of applications are enabled by the unique ability of IR spectroscopy to detect molecular composition of food materials using non-destructive sampling and rapid data collection. ML approaches can complement the current chemometric methods used for the analysis of IR spectroscopy data. Complementary to IR spectroscopy, fluorescence spectroscopy approaches rely on the photo-active properties of fluorophores in food systems and their relationship with changes in food quality and traceability~\citep{fluorescence}. Similarly, fluorescence properties have also been used to monitor the presence of bacteria in water samples~\citep{fluorescence_water}. However, due to significant interference between the food materials and bacterial components there has been limited applications of fluorescence spectroscopy in food safety. To address some of these limitations, this study evaluated the applications of Fluorescence EEM spectroscopy for food safety. EEM is a technique that allows for the complete, quantitative determination of the fluorescence profile of a given material and has been used for biomedical and material characterization applications~\citep{fluorescence_biomedical}.  Application of EEM spectroscopy including their integration with ML methods can address some of the key challenges in  application of fluorescence spectroscopy for food applications.  
 

\subsection{Related Work of Applying AL and SSL in Food Systems}

Research in food systems has adopted AL (a.k.a. optimal experimental design) to optimize non-ML model parameters, with the goal of reducing the number of experiments. It shows promising results of applying AL to applications such as determining partition coefficient in freeze concentration~\citep{freeze_al}, tuning micro-extraction in beer~\citep{beer_al}, identifying a rice drying model~\citep{rice_al}, and developing uniaxial expression of extracting oil from seeds~\citep{oil_al}. This paper differs from existing AL works in food science as we target general ML models while previous works are designed for specific and analytical models of few parameters. Similarly, SSL have successfully been used in food science problems such as determining tomato maturity~\citep{tomato_ssl} and tomato-juice freshness~\citep{tomato_juice_ssl}. To the best of our knowledge, this paper is the first work that extensively evaluates different AL and SSL approaches for the food science community. 




% \subsection{Active Learning in Batch Setting}

% We introduced the classical active learning setting in which a single data sample is selected at each iteration. In comparison, a batch sampling case of active learning chooses a subset of data samples at each iteration. [XXXX] It has  advantages when the number of data samples is large and deep convolutional neural networks are involved, considering (1) a single data sample is likely to have no statistically significant impact on the accuracy due to the local optimization methods, and (2) each sample in classical active learning requires a full training until convergence which makes it costly~\citep{activeLearningBatch18iclr}. However, the batch sampling case has the risky of selecting correlated samples in each interaction, without careful consideration [XXX].  

% \subsection{Active Learning in Streaming Setting}

% XXXXXXXXXXXXX

% \subsection{Active Learning for Sample Synthesis}

% In addition to selecting unlabeled samples for human annotation, active learning has been used to generate unlabeled samples. Compared to the traditional and manual sample synthesis by human experts, active learning is an essential component of automating sample searching, with the benefits of accelerated time frames and reduced resource wastes~\citep{drug_discovery_nature}. 
% For example,  active learning has been successfully applied by the medicine industry to discover antagonists for  dopamine $D_4$~\citep{drgu_d4} and CXC-chemokine~\citep{drgu_chemokine}, among the estimated range of $10^{30}$ -- $10^{60}$ drug-like molecules. 

% \subsection{Semi-supervised Learning Algorithm Selection}

% XXXXXXXXXXXXXXXXXXXXXXx


% \subsection{Other Practical Considerations}

% XXXXXXXXXXXXXXXXX

==> experimental_setup.tex <==
\subsection{Experimental Setup}
\label{sect:setup}


Given the same number of samples that can be annotated, we compare the ML model accuracy when different approaches of data annotation and model training are applied. 
We use the LightGBM multi-class classification model~\citep{lightgbm17nips} for the dosage classification dataset, and the linear Support Vector Classification (SVC) binary classification model~\citep{svm} for the pathogen detection dataset. We adopt 5-fold cross-validation for both datasets. Specifically, at each cross-validation round, the  training set and the validation set comprise the four-folds' samples and the remaining one-fold's samples, respectively. We use the training set for annotating a given number of samples and training, and apply the trained ML model to predict the validation set.
Note that the training set is assumed to be unlabeled at the beginning of each cross-validation, and the model is trained with different approaches (refer to Fig.~\ref{fig:scenario}). 
As with the conventional use of cross-validation,  the predictions for all samples are obtained by aggregating the predictions of the ML model for each validation set of the five cross-validations. 




%ML models' hyper-parameters (e.g., learning rate, regularization) affect the model training performance, and thus they need to be kept the same for all schemes to compare their performance fairly. \huanle{unfair for others}. 
To determine the hyper-parameters (e.g., learning rate, regularization) of ML models for a given number of labeled samples, we apply Optuna~\citep{optuna} to the passive learning approach and adopt the same hyper-parameters for all approaches. Therefore, the hyper-parameters favor the passive learning approach in our experiments.  With Optuna, we only need to provide reasonable ranges for hyper-parameters, and Optuna can identify the optimal hyper-parameters. We find that hyper-parameters from Optuna tend to have higher model accuracy than the default hyper-parameters. 





==> introduction.tex <==
\section{Introduction}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.9\textwidth]{image/scenario.png}
    \caption{Four approaches of data annotation and model training. (A) Passive learning. (B) Active learning. (C) Semi-supervised learning. (D) Hybrid of active learning and semi-supervised learning. }
    \label{fig:scenario}
\end{figure}


Rapid measurement and monitoring technologies are being developed for diversity of applications in the field of food science. The goal of these technologies are to development predictive relationships that can enable monitoring and improving  quality, safety and nutritional properties of food. Among these measurement approaches, spectroscopic analysis has been widely used for the analysis of food quality, safety, and nutritional properties. Despite significant potential, there are key barriers in translating these technologies to industrial applications. Among these barriers, development of predictive relationships between the measurements and properties of food systems is one of the key limitations. This limitation results due to complexity of food systems and the lack of comprehensive predictive models that can use rapid and simple measurements to predict complex properties in food systems. ML has shown significant potential to improve classification and prediction of these properties. However, the barriers to collect large datasets for ML applications still persists.


With the advances in computational capabilities and big data technologies, ML has been applied to a variety of agriculture and food related fields~\citep{ml_food, ml_agriculture, ml_water}. Before training an ML model, practitioners often need to collect labeled samples. Typically, it is convenient to collect unlabeled samples. In contrast, annotating samples is costly and time-consuming, as it often involves human inspection and in-field experiments. For example, to predict the vineyard yield, robot carrying cameras can be used to collect a large number of unlabeled images, but practitioners still need to manually process each image in order to assign appropriate labels to the images~\citep{vineyard_yield}. A prevailing practice is to randomly select a number of samples and label them via costly processes of in-field experiments and human annotation, and the ML model is trained only using the labeled samples. This approach results in poor data efficiency~\citep{burr_active_learning_book, semi_supervised_learning_book}. 
%In this paper, a scheme of data annotation and model training is designed to have a better data efficiency if the scheme uses fewer labeled samples to train an ML model with the same model accuracy. 


To improve data efficiency, we explore two advanced model training techniques: AL~\citep{burr_active_learning_book} and SSL~\citep{semi_supervised_learning_book}. Instead of randomly selecting unlabeled samples for annotation, AL selects samples for annotation based on how informative these samples are to the currently trained ML model. In comparison, SSL exploits unlabeled samples by assigning pseudo-labels to them and trains the ML model using both labeled and pseudo-labeled samples. 
Both AL and SSL have been successfully applied to many domains, such as drug discovery~\citep{al_drug, ssl_drug}, material science~\citep{al_material, ssl_material}, and systems biology~\citep{opex20nature,ssl_biology}.


In this paper, we study four approaches of data annotation and model training as illustrated in Fig.~\ref{fig:scenario}. (A) In the baseline passive learning approach, samples are randomly selected from the pool of unlabeled samples for annotation, and the ML model is trained only on the labeled samples. (B) In the AL approach (details in Sect.~\ref{sect:active_learning}), the selection of unlabeled samples is dependent on the currently trained ML model. In other words, AL selects the unlabeled samples that are most useful for training the ML model. Various sampling strategies are available, which quantify the usefulness of unlabeled samples based on different criteria. The ML model is trained only using the labeled samples. 
(C) In the SSL approach (details in Sect.~\ref{sect:semi-supervised_learning}),  unlabeled samples are randomly selected for annotation. Instead of training the ML model using only the labeled samples, SSL assigns pseudo-labels to the  unlabeled samples. The ML model is trained using both the labeled and the pseudo-labeled samples. Therefore, the number of training samples in SSL equals to the number of initial unlabeled samples. The methods of assigning pseudo-labels can be either related to the currently trained ML model (e.g., self-training) or rely only on the relationship among samples (e.g., label spreading). 
(D) In the hybrid approach that integrates AL and SSL, AL selects an unlabeled sample for annotation and SSL assigns pseudo-labels to the remaining unlabeled samples in each iteration. The ML model is trained using both labeled samples and pseudo-labeled samples. In this hybrid approach, AL and SSL interact with each other in the following manner. The sampling strategy in AL is dependent on the ML model, which is trained using labeled samples from human annotation and pseudo-labeled samples from SSL. Meanwhile, labeled samples from AL affect SSL regarding which samples are required for pseudo-annotation.  


% (1) \emph{Plasma Dosage Classification}. As an emerging nonthermal processing technology, plasma is highly effective in inactivating various types of food pathogens in solution as well as on food contact surfaces~\citep{plasma_review}. The dataset for plasma dosage classification was obtained by subjecting substrate to plasma treatment at various dosage levels and characterizing biochemical changes of substrate with Fourier-Transform Infrared Spectroscopy (FTIR). The data comprise aborbance intensities at various IR wavenumbers of the substrate under plasma treatment.
%We use the plasma dosage classification dataset to train a multi-classification ML model. (2) \emph{Foodborne Pathogen Detection}. Detection of the bacterial foodborne pathogen is one of the critical processes in the food and agricultural industry as it ensures the safety of food products before distribution and also reduces the risk of foodborne illness outbreak~\citep{pathogen_review}.  The dataset for pathogen detection was obtained by using bacteriophage for infection and lysis of the target bacterial pathogen in food samples. The fluorescence spectroscopy was then used to acquire the fluorescence Excitation Emission Matrices (EEM)~\citep{t7phage20chemical} of each sample. The data comprise fluorescence emission intensities at several pairs of excitation/emission wavelengths. We use the pathogen detection dataset to train a binary classification ML model. 





To evaluate different approaches for spectroscopic analysis in the food science field, we collect two datasets: plasma dosage classification and foodborne pathogen detection.
Atmospheric plasma technologies is being developed as a non-thermal processing technology to improve food safety and reduce impact on food quality and improve sustainability of food processing operations. One of the key challenges in applications of plasma technology is the rapid assessment of its efficacy in sanitation of food contact surfaces and food products. With this motivation, we are developing infra-red spectroscopy methods to aid in assessing dosimetry of plasma treatment. Similarly, rapid detection of the presence of foodborne pathogens is a critical unmet need in the food systems. In this direction, we are developing florescence spectroscopic methods based on molecular interactions between bacteriophages and their target bacteria to enable specific detection of bacteria.

%These spectroscopy methods illustrate examples of datasets to advance application of active learning and improve data efficiency for machine learning models
We apply different ML models for the multi-class classification task (plasma dosage classification) and the binary classification task (foodborne pathogen detection). 
Representative methods are considered for AL and SSL. 
%In particular, we cover uncertainty sampling and minimizing expected errors for AL, and self-training and label spreading for SSL. 
In the experiments, we adopt 5-fold cross-validation for both datasets. Our experimental results show that compared to the baseline passive learning approach, the number of labeled samples for the plasma dosage classification dataset is reduced by $\sim\!50\%$ using the hybrid approach, and the pathogen detection dataset benefits the most from the AL approach, with $\sim\!25\%$ fewer labeled samples required. The promising results demonstrate that AL and SSL based approaches of data annotation and model training are effective in improving data efficiency for  spectroscopy-based ML applications in food science. 




==> materials_and_methods.tex <==

\begin{table}[!t]
    \centering
    \begin{tabular}{c c}
        Notation & Meaning  \\\hline 
        \toprule
        $\theta$ & the currently trained ML model \\
        $\theta^+$ & an updated ML model by adding a new training sample \\
        $C$ & the number of classes for classification \\
        $x$ & a sample \\
        $y$ &  the label of the sample $x$ \\
        $x^*$ & the sample that has the maximum utility measure \\
        $y^*$ & the label of the sample $x^*$ \\
        $P_{\theta}(y|x)$ &  the probability that the sample $x$ belongs to the label $y$ under the model $\theta$ \\ $\hat{y}$  & the most likely label for the sample $x$, i.e., $\hat{y} = \argmax_y P_{\theta}(y|x)$ \\\hline 
    \end{tabular}
    \caption{Notations used in this paper. }
    \label{tab:notation}
\end{table}

\section{Materials and Methods}


In this section, we first provide preliminaries for AL in Sect.~\ref{sect:active_learning} and SSL in Sect.~\ref{sect:semi-supervised_learning}. Then, we explain our two datasets in detail in Sect.~\ref{sect:dataset}. Last, our experimental setup is given in  Sect.~\ref{sect:setup}. Table \ref{tab:notation} tabulates the notations that are used in this paper for quick reference. 

\input{active_learning}

\input{semi_supervised_learning}

\input{dataset}

\input{experimental_setup}




==> results.tex <==
\section{Results}


\begin{figure}[!t]
    \centering
    \centerline{
    \includegraphics[width=1\textwidth]{image/Sample_Illustration.png}
    }
    \caption{Demonstration of the samples selected in the passive learning approach and the active learning approach for the plasma dosage classification dataset. (A) Passive learning approach. (B) Active learning approach with the entropy-based uncertainty sampling. The 40 randomly selected samples for training an initial ML model are marked with ``*''. The next 10 samples are tagged with the order number.}
    \label{fig:sample_selection}
\end{figure}


We evaluate the four approaches of data annotation and model training using our two datasets. We warm start a LightGBM model using 40 randomly selected labeled samples for the dosage classification dataset and then apply different approaches. We run 10 experiments to average the results for the dosage classification dataset. Likewise, we first train a linear SVC model using 25 randomly selected labeled samples for the pathogen detection dataset before applying different approaches. 20 experiments are conducted to average the results for the pathogen detection dataset. Since we adopt the 5-fold cross-validation, the maximum number of samples for training in each cross-validation is 90 for the dosage classification task and 56 for the pathogen detection task. 


\subsection{Results of the Active Learning Approach}


We first demonstrate the order of samples selected for annotation in the passive learning approach and the AL approach. Principal Component Analysis (PCA)~\citep{pca} is applied to project the high-dimensional samples into two components for visualization. Fig.~\ref{fig:sample_selection}
illustrates a trace for the passive learning approach and the AL approach for the dosage classification dataset, respectively. 
%As we can see, the selected samples in the passive learning scenario can be near the center of one class. In this region, the currently trained ML model has already been able to classify them correctly, and thus, these samples do not help the model training. 
As Fig.~\ref{fig:sample_selection}(A) illustrates, the selected samples in the passive learning can be close to each other and also near the center of the class (e.g., samples 2, 3, and 7), which are less likely to improve the ML model accuracy. In comparison, as Fig.~\ref{fig:sample_selection}(B) shows, the selected samples in the AL approach are close to the boundaries of different classes. In these boundary areas, the ML model is difficult to classify. Thus, training with the samples selected by AL is more likely to increase the ML model accuracy. 


\begin{figure}[!t]
    \centering
    \centerline{
    \includegraphics[width=0.9\textwidth]{image/pool_based_active_learning.png}
    }
    \caption{The ML model performance versus the number of labeled samples in the AL approach. The first row and the second row show the results for the dosage classification dataset and the pathogen detection dataset, respectively. (A) and (C): uncertainty sampling based on least confident and entropy; (B) and (D) minimizing expected prediction error and expected log-loss error based sampling.}
    \label{fig:pool_active_learning}
\end{figure}

In the rest of the experiments for the AL approach, we consider (1) uncertainty sampling methods based on least confident and maximum entropy, and (2) minimizing the expected prediction error and the expected log-loss error.
Fig.~\ref{fig:pool_active_learning} plots the ML model accuracy versus the number of labeled samples. The first row and the second row show the model performance for the dosage classification and the pathogen detection datasets, respectively. We show the standard deviation in shaded colors.  As Fig.~\ref{fig:pool_active_learning}(A) illustrates, the AL approach with uncertainty sampling obviously improves the data efficiency for the dosage classification dataset: $\sim\!70$ labeled samples achieve approximately the same model accuracy of using all 90 labeled samples. Fig.~\ref{fig:pool_active_learning}(B) shows that the sampling strategies of minimizing expected errors do not perform as well as the uncertainty-based sampling strategies. Since the current model accuracy is only $\sim\!70\%$, the calculated expected errors are inaccurate. In comparison, the uncertainty sampling identifies samples of high uncertainty for the currently trained ML model, which is irrespective of the model accuracy. Nonetheless, the sampling strategies of minimizing expected errors are still slightly better than the passive learning approach for the dosage classification dataset.  
For the pathogen detection dataset as shown in Fig.~\ref{fig:pool_active_learning}(C) and Fig.~\ref{fig:pool_active_learning}(D), we observe similar performance comparisons between the AL approach and the passive learning approach. Uncertainty-based AL greatly reduces the number of labeled samples for training ML models, with 25\% less data required ($\sim\!40$ labeled samples achieve the similar accuracy of using all 56 samples). The sampling strategies of minimizing expected errors are comparable to the passive learning approach. 


From the experiment results of the AL approach, we can draw the following conclusions. 
(1) The AL approach can obviously improve data efficiency for training ML models if a suitable sampling strategy is applied. For example, uncertainty-based sampling performs well for both datasets. (2) The AL approach does not guarantee a superior performance than the passive learning approach. For example, sampling strategies of minimizing expected errors depend on the current ML model accuracy to calculate the expected errors, which does not perform well if the current ML model has low prediction accuracy. Nonetheless, we do not see a noticeable degradation of model accuracy when applying the AL approach. 
 

\subsection{Results of the Semi-supervised Learning Approach}


\begin{figure}[!t]
    \centering
    \centerline{
    \includegraphics[width=0.9\textwidth]{image/semi_supervised_learning.png}
    }
    \caption{The ML model accuracy versus the number of labeled samples in the semi-supervised learning approach. The first row and the second row show the results for the dosage classification dataset and the pathogen detection dataset, respectively. (A) and (C): self-training based on maximum confident and minimum entropy; (B) and (D): label spreading based on kNN kernel and RBF kernel.}
    \label{fig:semi_supervised_learning}
\end{figure}


SSL exploits unlabeled samples by assigning pseudo-labels to them and then trains the ML model using both labeled and pseudo-labeled samples. In the evaluation of the SSL approach, we consider self-training and label spreading. We set the number of neighbors in the kNN kernel to 7 and the $\sigma$ in the RBF kernel to 0.1 for both datasets. 



Fig.~\ref{fig:semi_supervised_learning} plots the ML model accuracy versus the number of labeled samples in the SSL approach. The first row and the second row show the model performance for the dosage classification dataset and the pathogen detection dataset. We visualize the standard deviation in shaded colors.  Fig.~\ref{fig:semi_supervised_learning}(A) and Fig.~\ref{fig:semi_supervised_learning}(B) clearly show that the SSL approach can improve the model accuracy for the dosage classification dataset when the number of labeled samples is small, e.g., less than 50 labeled samples. As expected, the SSL approach converges to the passive learning approach when most samples are labeled (e.g., 70 labeled samples onward). For the pathogen detection dataset, however, the semi-supervised learning approach has almost the same performance as the passive learning approach, as Fig.~\ref{fig:semi_supervised_learning}(C) and Fig.~\ref{fig:semi_supervised_learning}(D) illustrate. The pathogen detection dataset does not benefit from the SSL approach is probably because its samples are not well-clustered, as indicated in Fig.~\ref{fig:dataset}(E). The cluster assumption, which is often included as a necessary condition for SSL, requires that data samples from the same cluster belong to the same class~\citep{semi_supervised_learning_book}.


From the results of the SSL approach, we can make the following conclusions. (1) When the number of labeled samples is small compared to the total number of samples, the SSL approach has the significant potential to improve data efficiency for training ML models (e.g., label spreading for the dosage classification dataset). (2) The SSL approach converges to the passive learning approach when most samples are labeled. (3) The SSL approach does not work well when the samples are not well-clustered due to the necessary condition of the cluster assumption (e.g., the pathogen detection dataset). Nevertheless, we do not see an apparent model performance degradation using the SSL approach compared to the passive learning approach. 



\subsection{Results of the Hybrid Approach}


\begin{figure}[!t]
    \centering
    \centerline{
    \includegraphics[width=0.9\textwidth]{image/combine_all.png}
    }
    \caption{The ML model accuracy versus the number of labeled samples in the hybrid approach.  (A) Dosage classification dataset. (B) Pathogen detection dataset. }
    \label{fig:combine}
\end{figure}


We measure the performance of the hybrid approach using the entropy-based uncertainty sampling for AL and RBF-based label spreading for SSL. The $\sigma$ in the label spreading is set to 0.01 for both datasets. 


Fig.~\ref{fig:combine} shows the ML model accuracy for the hybrid approach, where (A) is for the dosage classification dataset and (B) is for the pathogen detection dataset. Fig.~\ref{fig:combine}(A) illustrates that, compared to the AL approach (Fig.~\ref{fig:pool_active_learning}(A)(B)) and the SSL approach (Fig.~\ref{fig:semi_supervised_learning}(A)(B)), the hybrid approach for the dosage classification dataset further improves data efficiency for the ML model training. Specifically, $\sim\!45$ labeled samples achieve the same accuracy of using all 90 labeled samples, reducing the number of labeled samples by $50\%$. However, for the pathogen detection dataset, the hybrid approach has approximately the same performance as the passive learning approach (Fig.~\ref{fig:combine}(B)). As we previously discussed, the pathogen detection dataset is not well-clustered, and thus SSL does not work well. The benefit of AL is suppressed by integrating it with SSL, indicating the interaction between AL and SSL is inherently complicated. 


From the results of the hybrid approach, we make the following observations. (1) The hybrid approach can provide supreme performance, which greatly improves the data efficiency of ML model training (e.g., the dosage classification dataset). (2) The hybrid approach does not guarantee better performance than the AL approach and the SSL approach. For the pathogen detection database, the AL approach works better than the hybrid approach. Nevertheless, we do not see a noticeable model performance degradation using the hybrid approach compared to the passive learning approach. 


==> semi_supervised_learning.tex <==
\subsection{Semi-Supervised Learning: A Primer}
\label{sect:semi-supervised_learning}


\begin{algorithm}[!t]
\SetAlgoLined
$\mathcal{U}$: set of unlabeled samples $\{x^{(u)}\}_{u=1}^U$ \\
$\mathcal{L}$: set of labeled samples $\{\langle x, y\rangle^{(l)}\}_{l=1}^L$

% \For{$t = 1, 2, ...$ }{
\While{$\mathcal{U} \text{ is not empty}$}{
    $\theta = \textbf{train}(\mathcal{L})$\\
    select  $x^* \in \mathcal{U}$, the most confident sample according to model $\theta$\\
    obtain the pseudo-label of $x^*$ by applying the current model $\theta$ to it, i.e., $\theta(x^*)$\\
    remove  $x^*$ from $\mathcal{U}$  and add  $\langle x^*, \theta(x^*) \rangle$ to $\mathcal{L}$
}
\caption{Self-training based semi-supervised learning.}
\label{alg:self_train}
\end{algorithm}




SSL can be applied to exploit unlabeled samples. Typically, an SSL algorithm converts unlabeled samples to pseudo-labeled samples and then fine-trains the ML model using both labeled and pseudo-labeled samples. SSL can be categorized into inductive methods and transductive methods~\citep{semi_supervised_learning_survey20ML}. We introduce  self-training~\citep{selfTraining} and label spreading~\citep{labelSpreading}, which are representative methods from these two categories, respectively. 

\subsubsection{Self-Training based Semi-Supervised Learning}

In self-training based method, the currently trained ML model is applied to pseudo-annotate the unlabeled samples~\citep{selfTraining}. 
%The ML model is re-trained using both the labeled samples and the pseudo-labeled samples. 
Self-training methods assume that the prediction of the current model tends to be correct, and thus the model can be further fine-trained by leveraging more training samples.


Algorithm \ref{alg:self_train} shows the workflow of self-training based SSL.
It differs from the AL workflow (Algorithm \ref{alg:pool-based}) in two main parts. 
(1) The unlabeled sample $x$ is pseudo-labeled by the model itself, i.e., $\theta(x^*)$, in self-training, whereas it is human-annotated, i.e., the ground-truth label $y^*$, in AL (line 6 in Algorithm \ref{alg:self_train} versus line 6 in Algorithm \ref{alg:pool-based}). (2) The most confident unlabeled sample is selected in self-training. In contrast, the most uncertain unlabeled sample is chosen in AL (line 5 in Algorithm \ref{alg:self_train} versus line 5 in Algorithm \ref{alg:pool-based}). Self-training selects the most confident unlabeled sample to mitigate the error propagation of pseudo-annotation since the model $\theta$ is consecutively trained on the pseudo-labeled samples. In contrast, AL selects the model's most confusing unlabeled sample for human annotation so that the model can correctly classify misleading samples. The whole process of unlabeled sample selection, pseudo-annotation, and model training is repeated until all the unlabeled samples are pseudo-annotated (line 3). At that time, the model has been trained on all labeled and pseudo-labeled samples.


\subsubsection{Label Spreading based Semi-Supervised Learning}


Label spreading based SSL typically adopts a graph structure, where the vertices are the samples (both labeled and unlabeled) and edges exist between neighbor vertices~\citep{labelSpreading}. The edge weight between two vertices represents the similarity of the corresponding two samples. The goal of label spreading is to assign pseudo-labels to the vertices of unlabeled samples. The labels of $x_i$ and $x_j$ are likely to be the same if the edge weight $w_{ij}$ between them is large. There are two mainstream methods to define the graph structure and the edge weights:
\begin{itemize}
    \item \emph{Fully Connected Graph}~\citep{ssl_graph}. In this graph, all vertices are connected with other vertices, and the edge weight $w_{ij}$ between $x_i$ and $x_j$ is calculated as 
\begin{equation}
    w_{ij} = \exp{(-\frac{||x_i - x_j||^2}{2\sigma^2})}
\end{equation}
where $||x_i - x_j||$ is the Euclidean distance between sample $x_i$ and sample $x_j$, and $\sigma$ controls the decreasing rate of the weight over the distance. The edge weight  $w_{ij}$ is 1 when $x_i = x_j$, and 0 when $x_i$ is far from $x_j$. This weight representation is also called Radial Base Function (RBF) kernel or Gaussian kernel. 


\item \emph{k-Nearest-Neighbor (kNN) Graph}~\citep{ssl_graph}. In the kNN graph, each vertex is connected to its $k$ nearest vertices. If sample $x_i$ and sample $x_j$ are connected, the edge weight $w_{ij}$ is 1; otherwise, $w_{ij}$ is 0. The kNN graph automatically adapts to the density of samples: in dense regions, the radius of the kNN neighborhood is small, while in sparse regions, the radius is large. 

\end{itemize}

The probability of the label for each unlabeled sample is obtained once the graph is converged~\citep{labelSPread}. Then, each unlabeled sample is assigned to the label of the highest probability at once. Afterward, the ML model is re-trained using all samples (labeled and pseudo-labeled).



